Model Checking Software Programs with First Order Logic Specifications using AIG Solvers

Static verification techniques leverage Boolean formula satisfiability solvers such as SAT and SMT solvers that operate on conjunctive normal form and first order logic formulae, respectively, to validate programs. They force bounds on variable ranges and execution time and translate the program and its specifications into a Boolean formula. They are limited to programs of relatively low complexity for the following reasons. (1) A small increase in the bounds can cause a large increase in the size of the translated formula. (2) Boolean satisfiability solvers are restricted to using optimizations that apply at the level of the formula. Finally, (3) the Boolean formulae often need to be regenerated with higher bounds to ensure the correctness of the translation. We present a method that uses sequential circuits, Boolean formulae with memory elements and hierarchical structure, and sequential circuit synthesis and verification frameworks to validate programs. (1) Sequential circuits are much more succinct than Boolean formulae with no memory elements and preserve the high-level structure of the program. (2) Encoding the problem as a sequential circuit enables the use of a number of powerful automated analysis techniques that have no counterparts for other Boolean formulae. Our method takes an imperative program with a first order logic specification consisting of a precondition and a postcondition pair, and a bound on the program variable ranges, and produces a sequential circuit with a designated output that is true when the program violates the specification.

==> NoNewlineAfterSubSubSection.tex <==
\makeatletter
\renewcommand\subsubsection{\@startsection{subsubsection}{3}{\z@}%
  {-3.25ex\@plus -1ex \@minus -.2ex}%
  {-1.5ex \@plus -.2ex}% Formerly 1.5ex \@plus .2ex
  {\normalfont\normalsize\bfseries}}
\makeatother


==> arrays.tex <==
%% Arrays

\begin{figure}[bt]
 \centering
 \resizebox{0.4\textwidth}{!} {
     \input{figs/arrayaccess.pdf_t}
 }
 \caption{array access using a multiplexer}
 \label{f:arrayaccess}
\end{figure}

Arrays in CG2SC are represented at the circuit level by as a set of 
latches where each $n$ latches 
correspond to one element of the array, with
$n$ being the bound on the variables' size. Arrays that have a pre-defined 
size, i.e. a constant size are created to have their size equal to the 
assigned size. Arrays having a variable size or with no specified size 
(i.e. dynamic arrays) are assigned to a size limit, this limit being 
pre-assigned by the user, and its default value is limited by the amount
of memory that the underlying system can support. Typically this limit 
is to be $2^{10}$ elements per array.
In total, the number of latches needed to represent an array in the 
resulting sequential circuit is given by the following equation:
\begin{equation}
 numLatches = size \times bound
\end{equation}
where $numLatches$ is the number of latches needed, $size$ is the size
of the array and $bound$ is the bound on each variable. 

Accessing arrays elements (i.e. reading data from an array) is a simple 
operation that can be provided with the use of a large multiplexer.
This multiplexer will have a number of choices equal to the size of the 
array, and will be controlled by the appropriate index given in the 
array access statement.  
As an example, the statement \texttt{x = a[i]} will create a multiplexer
spanning all the element of array \texttt{a}, and controlled 
by the index \texttt{i}. The output of the multiplexer will go into 
the next state function of the variable \texttt{x}, and at the 
appropriate clock cycle, it will be passed to the actual value of 
\texttt{x}. Figure~\ref{f:arrayaccess} shows a diagram of the described 
operation.  

%% writing to an array element
Writing to an array element (i.e. assigning a value to an array element) 
is a more complexe operation. It cannot be solved by using a simple 
demultiplexer in a similar way to what we have in the reading phase. The 
main source of the complexity arises from the fact that we need to maintain
the same value at any latch that is not involved in the writing 
operation. In other words, an array element that is not being written 
should maintain a constant value, which is not achievable by using
a demultiplexer. 

In order to overcome this complexity, we decided to add for each element 
in the array its own index value. Therefore the first element in the array 
will have the index 0, the second element the index one and so on until we 
reach the last element which will have the index $n-1$. Subsequetely, at
each write to an array element, we create a set of binary multiplexers, 
one for each element. The inputs to the multiplexer are the current value
of the array element, and the new value to be written. The control for the
mux will be a comparison between the index in the write statement and 
the index of each array element. This operation is actually similar to the
following for loop:
\begin{Verbatim} [fontsize=\relsize{-2}, numbersep=4pt, numbers=left]
for (int i = 0; i < size; i++) {
    if (i == index)
        a[i] = expression;
}
\end{Verbatim}
with the exception that all iteration of this loop will be occuring at the
same clock cycle. In this way, we can maintain the value of the array 
elements that are not involved in the write operation, while only 
the ones that do match the write index will have their value overwritten. 


==> cases.tex <==
%% searching studies with CBMC
The programs $\Pm_1$ and $\Pm_2$ in Figures~\ref{fig:linearsearch} and~\ref{fig:binarysearch}
show the linear search and binary search algorithms annotated with appropriate
preconditions and postconditions, respectively. The precondition in $\Pm_1$ ensures that 
the provided size $n$ is valid, \ie positive and smaller than the largest allowed array size. 
The precondition in $Pm_2$ checks that the provided size $n$ is valid and that the 
array $a$ is sorted in ascending order. 
The postcondition in both $\Pm_1$ and $\Pm_2$ 
checks that when the returned index $rv$ is between 0 and the size $n$, then 
array element at the index, $a[rv]$, is equal to the element $e$ to search for. It also 
checks that when $rv$ is invalid, the element $e$ is not present in the 
array $a$. 

We use \psqtool{} and CBMC to verify that the programs $\Pm_1$ and $\Pm_2$ satisfy the 
precondition-postcondition pairs provided. We make use of the assume statement \cci{\_\_CPROVER\_assume}
in CBMC to implement the preconditions, and we encode the quantifiers as while loops. 
In \psqtool{}, we use the dedicate property grammar and the FOL support to write the specifications. 
We implement the check $precondition \implies postcondition$ as an assertion statement
in CBMC.

\begin{figure}[bt]
\begin{Verbatim}[fontsize=\relsize{-1.0}, numbersep=4pt,numbers=left]
int ls (int [] a, int e, int n) {
  @pre ls {0 <= n && n <= MAX_ARRAY_SIZE}
  int i = 0;
  while (i < n) {
    if (a[i] == e)
      return i;
    i = i + 1;  
  }
  return -1;
  
  @post ls { (rv >= 0 && rv < n) -> (a[rv] == e) &&
    (rv == -1) -> (forall(int i:[0..n-1]) {a[i] != e})
  }
}
\end{Verbatim}
\caption{The linear search algorithm with pre and post conditions}
\label{fig:linearsearch}
\end{figure}

\begin{figure}[bt]
\begin{Verbatim}[fontsize=\relsize{-1.0}, numbersep=4pt,numbers=left]
int bs (int [] a, int e, int n) {
  @pre bs {0 <= n && n <= MAX_ARRAY_SIZE && isSorted(a,n)}
  int low = 0, high = n -1;
  while (low < high) {
    int mid = (low + high) >> 1;
    if (a[mid] < e) {
      low = mid + 1;
    } else {
      high = mid;
    }
  }
  if ((low == high) && (a[low] == el)) {
    return low;
  } else {
    return -1;
  }
  
  @post bs { (rv >= 0 && rv < n) -> (a[rv] == e) &&
    (rv == -1) -> (forall(int i:[0..n-1]) {a[i] != e})
  }
}

isSorted(int [] a, int n) = forall(int i:[0..n-2]) {
  a[i] <= a[i+1]
}
\end{Verbatim}
\caption{The binary search algorithm with pre and post conditions}
\label{fig:binarysearch}
\end{figure}

We compare the results obtained from \psqtool{} and CBMC in terms of the problem size and
verification time. The problem size is defined as the number of variables and clauses 
in the generated CNF formulae in CBMC, and the number of latches, AND gates and logic levels
in the generated AIGs in \psqtool{}. We report on the size of the generated formulae and AIGs
after performing optimization and reduction steps in both CBMC and \psqtool{}. We compare 
the time taken by both tools to perform all of the required steps to return a decision, 
including both optimization and verification.
Since CBMC supports only $16$, $32$ and $64$ bits scalars, we use the size of the input
array $a$ as the variable to change between different settings of the programs $\Pm_1$
and $\Pm_2$. We set a time-out limit of $30$ minutes and do not set a limit on the 
amount of memory the program can use (up to the machine's physical limit).

Note that in the addition to the above, CBMC requires users to provide an {\em unwinding
limit}. This limit is used by CBMC to unroll loops in the input programs $\Pm_1$ and $\Pm_2$.
We use an unwinding limit of $2\times array\_size$ for our experiments and we enable 
the CBMC unwinding assertions. \psqtool{} does not require any unwinding limit since
it does not perform unrolling, it uses the program counter to execute the loops infinitely 
many times using the same AIG. 

Table~\ref{tb:cbmc_compare} shows the results of using \psqtool{} and CBMC to verify the 
programs $\Pm_1$ and $\Pm_2$ for different sizes of the input array $a$, shown in the 
column {\em size}. The columns {\em Vars} and {\em Clauses} report on the size of the
CNF formula generated by CBMC in terms of the number of variables and clauses, respectively. 
The columns {\em lat}, {\em and} and {\em lev} show the size of the generated AIG by \psqtool{}
in terms of the number of latches, and gates and logic levels, respectively. The last two columns
show the time taken by \psqtool{} and CBMC to perform both reduction and verification. 
The {\em Time-out} entry indicates that the tool reached the time out limit before 
returning a conclusive result about the verification problem.

\input{table_comparison}

The results show that \psqtool{} is able to verify the linear search program $\Pm_1$ 
for sizes much higher than those provided by CBMC. For array size of $15$ and above, \psqtool{}
is able to efficiently generate the AIG, and call ABC to reduce and verify it, while CBMC
reached the time out limit without giving any decision. Also, the size of the generated AIG 
by \psqtool{} is always smaller than the size of the CNF formula generated by CBMC.
For example, for an array size of $15$, CBMC's CNF formula contains $9112$ variables
and $34496$ clauses, while \psqtool{}'s AIG has $119$ bit registers and $1116$ AND gates.
This clearly shows the advantage that the program counter encoding provides over 
loop unrolling. 

For the binary search program ($\Pm_2$), both tools show similar performance for sizes of $3$, $7$
and $15$. \psqtool{} outperforms CBMC for a bound of $63$ since CBMC reached the time out limit
while \psqtool{} was able to verify the program in $1152$ seconds. Similarly to $\Pm_1$, 
the size of the generated AIGs by \psqtool{} is orders of magnitudes smaller than the size of the 
generated CNF formulae by CBMC. For example, for a size of $63$, the number of variables  
in the generated AIG is $99\%$ smaller than the number of variables in the generated CNF formula.


==> cmdComment.tex <==
\def\parsearg #1{\let\next=#1\begingroup\obeylines\futurelet\temp\parseargx}

\def\parseargx{%
\ifx \obeyedspace\temp \aftergroup\parseargdiscardspace \else%
\aftergroup \parseargline %
\fi \endgroup}

{\obeyspaces %
\gdef\parseargdiscardspace {\begingroup\obeylines\futurelet\temp\parseargx}}

\gdef\obeyedspace{\ }

\def\parseargline{\begingroup \obeylines \parsearglinex}
{\obeylines %
\gdef\parsearglinex #1^^M{\endgroup \next {#1}}}

\def\flushcr{\ifx\par\lisppar \def\next##1{}\else \let\next=\relax \fi \next}


\def\comment{\parsearg \commentxxx}
\def\commentxxx #1{}



==> ctooneloop.old.tex <==

\begin{algorithm}[tb]
\begin{algorithmic}[1]
\State {\bf Input:} \psqlanguage~ program \Pm, $entry\_statement$
\State {\bf Output:} \oneloop~ program $\mathcal{C}$
\State 
\State // build the initialization list
\State init\_list $[ ]$
\ForAll { $v \in V$}
 \If{used\_before\_assigned($v$)}
  \State init\_list.insert ($``v = free\_inputs"$)
 \EndIf
\EndFor
\State init\_list.insert ($``pc = label(entry\_statement)"$)
\State
\State // build the next state list for variables
\State next\_state\_list $[ ]$
\ForAll {$v \in V$}
 \State $next_v = ``v = "$
 \ForAll {Assignment statement $s$ such that $target(s) = v$}
  \State $next_v += ``(pc==label(s))? ~expression(s) : "$
 \EndFor
 \State $next_v += ``v"$
 \State next\_state\_list.insert $(next_v)$
\EndFor
\State 
\State // build the next state for the program counter
\State $n_{pc} = ``pc = "$
\ForAll {statement $s$}
 \If {is\_conditional\_statement ($s$)}
   \State $n_{pc} += ``(pc==label(s))?~ (condition(s)?~then(s) : else(s)) :"$
 \ElsIf {is\_loop\_statement ($s$)}
   \State $n_{pc} += ``(pc==label(s))?~ (condition(s)?~body(s):next(s)) :"$ 
 \ElsIf {is\_function\_call(s)}
   \State $f_d :=$ function\_declaration\_of $(s)$
   \State $n_{pc} += ``(pc==label(s))?~ (body(f_d)) :"$
 \ElsIf {is\_return\_statement (s)}
   \State $f_d :=$ function\_declaration\_of $(s)$
   \State $n_{pc} += ``(pc==label(s))?~(return(call(f_d))) :"$
 \Else 
   \State $n_{pc} += ``(pc==label(s))?~(next(s)) :"$
 \EndIf
\EndFor
\State next\_state\_list.insert $(n_{pc})$
\end{algorithmic}
\caption{\psqlanguage~to \oneloop~transformation algorithm}
\label{algo:psqtoettrans}
\end{algorithm}

Algorithm~\ref{algo:psqtoettrans} shows the procedure used 
in \psqtool~to translate a preprocessed \psqlanguage~program \Pm
with a set of variables $V$ and an initial entry statement, into an \oneloop~program 
$\mathcal{C}$, to be used for the synthesis of the equisatisfiable 
AIG. Intuitively, the wire declarations, variable definitions and wire definitions are directly moved from 
 \Pm to their corresponding blocks in \aigcircuit.
Additionally, in order to model time, \psqtool~adds a new
scalar variable to the program \Pm, the {\em program
counter} \cci{pc}. This variable is key to avoid 
inlining functions and unrolling loops. It is used to 
ensure the proper sequencing of the statements of \Pm;
the current value of the \cci{pc} variable defines which 
statement is to be execute. For example, reassigning the 
value of \cci{pc} to the starting point of a loop's body
allows \psqtool~to make use of the same code block (thus
the same AIG) to execute a single loop infinitely many 
times. 

The algorithm starts by building the initialization list
of \aigcircuit. It assigns the program counter variable
\cci{pc} to the label of the entry statement of \Pm.
Then for each variable $v \in V$ that is used before
being assigned (i.e. used with an undefined value), it 
assigns $v$ to a set of free inputs (AIG primary inputs)
who's values are to be set by the ABC AIG solver. 
Note that since variables can be initialized at different
points in the program (and not necessarily at the starting
point of the algorithm), we delay their
initialization step 
into the \cci{next} block, where these variables
will get their initial value at the appropriate \cci{pc}
value.

Subsequently, the algorithm moves to building the
\cci{next} state block of \aigcircuit. For each 
variable $v \in V$, and for each assignment statement 
$s$ such that $target(s)=v$, the next state of $v$ will
be $expression(s)$ iff $pc == label(s)$. If at a given 
statement label, $v$ is not being assigned, it retains
its current value. For example, consider the 
following assignment
statements for $v$:
\begin{Verbatim}[fontsize=\relsize{-1.0}, numbersep=4pt,numbers=left]
(l1): x = 1;
(l2): x = 3;
(l3): x = 5;
\end{Verbatim}
The algorithm builds the next state function of $x$ as 
the following statement
\begin{Verbatim}[fontsize=\relsize{-1.0}, numbersep=4pt,numbers=left]
x = (pc == l1)? 1 : (pc == l2)? 3 : (pc == l3)? 5 : x;
\end{Verbatim}

After traversing all variables of \Pm, the algorithm
then builds the next state assignment for the program counter.
At a given statement $s$, the default behavior of the \cci{pc} is to move from the current label $label (s)$
to the label of the statement that directly follows
$s$, i.e. $next(s)$. 
Only control statements such as conditional statements, 
loop statements, function call statements and return 
statements are allowed to alter the default behavior of 
\cci{pc}.

Conditional statements alter the value of the 
program counter based on the evaluation of their
conditional expression. Consider a conditional statement
$s$ and let $e = condition(s)$. When \cci{pc} is at 
$label(s)$, its next value is either the label 
of the first statement in then \cci{then} branch of $s$
if $e$ evaluates to $true$, or to the first
statement in the \cci{else} branch of $s$ otherwise. 
Therefore at $label(s)$, the next state of the \cci{pc}
is defined as $(e)?~ then(s) : else(s)$.

Similarly, loop statements move the program counter
into their body when their conditional expression evaluates
to $true$, and to their next statement once it is $false$.
Consider a loop statement $s$ and let $e = condition(s)$.
At $label(s)$, the next state of \cci{pc} is defined
as $(e)?~ body(s):next(s)$. Note that according to the 
\psqlanguage, the loop statement block is considered 
as a single statement, and thus the next statement 
to follow $s$ would be the first statement outside its 
body, i.e. its exit point. Additionally, for the last
statement in the body of the loop, its next statement
is defined as the loop statement itself. This ensure that
once the \cci{pc} reaches that last statement in the 
loop, it once again evaluates its condition in order to
determine whether to exit or stay in the loop.  

Finally, function call statements and return statements 
redirect the program counter into the body of the function 
and to the first statement after the call, respectively. 
Note that for a non-recursive function, there is at most
one active function call at a time, therefore it is easy
to track the label at which the program counter 
should return to.
For a recursive function, we maintain a stack of function calls and redirect the control to statement after the 
call that is on top of the stack. 

\subsubsection*{Post-processing}
After constructing the \oneloop~program \aigcircuit,
\psqtool~employs a last post-processing step to resolve 
array accessing. Given an array access expression 
$a[i]$ where $a$ is an array and $i$ is an index, resolving
this access expression is to transform it into an array
access where the index is constant. An array access 
expression with a constant index is handled as a regular 
register variable in \aigcircuit. 

The first part of algorithm~\ref{alg:resolv_target_exp} 
shows the post
processing of a reference to an array access expression 
$e$. The algorithm pushes the variable index $i$ outside
of the array access by creating a set of checks for the 
value of $i$ at each possible index of the array $a$, and
returning the appropriate array element accordingly.

The second part of algorithm~\ref{alg:resolv_target_exp} 
shows the 
post processing of statement $s$ where $target(s)$
is an array access of the form $a[i]$. Since this 
assignment statement can be to any of the elements of the 
array $a$, as dictated by the value of $i$, the algorithm
creates an assignment statement for each possible 
element of $a$. This ensure that only the correct element
get assigned to the value of $expression(e)$ by creating
a check for $i$ at each possible index of the array.  

Figure~\ref{fig:trans:arrays} shows an \oneloop~program 
\aigcircuit~that contains array access assignments and 
references. Post-processing transforms the assignment
statement on line 14 of the program \aigcircuit into 
assignment statements over all the elements of the
array $a$, with added checks on the value of the index
$i$. Also post-processing replaces the expression $b[k]$ 
in the right hand side of the assignment statements 
with the expression $(k==0)?~b[0] : b[1]$. This expression
checks on the value of $k$ for all possible indices to the 
array $b$ and returns the corresponding
element. 

\begin{figure}[bt]
\centering
\begin{tabular}{p{0.33\textwidth}|p{0.01in}p{0.33\textwidth}}
\begin{Verbatim}[fontsize=\relsize{-2.5}, numbersep=4pt,numbers=left,
frame=topline, framesep=4mm, label=\fbox{Program \aigcircuit}]
int a [2];
int b [2];
int i, k;
@dotogether {
  a[0] = free_inputs;
  a[1] = free_inputs;
  i = free_inputs;
  k = free_inputs;
  b[0] = free_inputs;
  b[1] = free_inputs;
}
 
@dotogether {
  a[i] = (pc == l1)? b[k] : a[i];
}
\end{Verbatim}
& &
\begin{Verbatim} [fontsize=\relsize{-2.5}, numbersep=4pt,numbers=left,
frame=topline, framesep=4mm, label=\fbox{\aigcircuit~after
post-processing}]
int a [2];
int b [2];
int i, k;
@dotogether {
  a[0] = free_inputs;
  a[1] = free_inputs;
  i = free_inputs;
  k = free_inputs;
  b[0] = free_inputs;
  b[1] = free_inputs;
}
 
@dotogether {
  a[0] = (i == 0)? 
           ((pc == l1)? ((k == 0)? b[0] : b[1]) : a[0]) 
           : a[0];
  a[1] = (i == 1)? 
           ((pc == l1)? ((k == 0)? b[0] : b[1]) : a[1]) 
           : a[1];
}
\end{Verbatim}
\end{tabular}
\caption{Post processing of a \oneloop~\aigcircuit}
\label{fig:trans:arrays}
\end{figure}


\begin{algorithm}[h!]
 \begin{algorithmic}[1]
  \State // array access on right hand side
 \State {\bf Input:} Array access expression $e$
  \State {\bf Output:} Array access expressions $e'$ with 
  constant indexing
  \State $a := base(e)$
  \State $i := index(e)$
  \State $N := size(a) - 1$
  \For{$j \in 0 \ldots N-1$}
   \State $e' += (i == j)?~ a[j] :$
  \EndFor
  \State $e' += a[N]$
  \State
  \State // array access on left hand side
  \State {\bf Input:} Statement of the form $a[i] = e$, 
  $e$ is an expression
  \State {\bf Output:} A list of statements where all array accesses have a constant index 
  \State List\_of\_statements $[ ]$
  \State $N := size(a) - 1$
  \For{$j \in 0 \ldots N-1$}
   \State List\_of\_statements.insert $(a[j] = (i == j)?~ e : a[j])$
  \EndFor
 \end{algorithmic}
 \caption{Array access resolving algorithm}
 \label{alg:resolv_target_exp}
\end{algorithm}



==> func_control_flow.tex <==
%% functions control flow
Each function should maintain a set of control-flow related information, in order to 
execute correctly and prepare for a correct translation. This set, in addition to data-flow
information, contains the following:
\begin{enumerate}
 \item A scalar counter that is used as a reference counter for dealing with passing arrays
by reference as described in section~\ref{s:func_data_flow}. It is initialized to zero
and increment at each function call, giving each one of these calls, and thus each 
array argument a unique identifier. 
 \item Each function call will save its own local return program counter, which represents
the address at which the program counter should return to after executing the function
body. The reason for having a local return PC for each function call is to provide support
for recursion, which will be explained in Section~\ref{s:func_recursion}.
 \item Each function declaration (i.e. function body) will have a unique return program
counter. It has the same functionality as the one that is local for each function call, 
with the difference that it is unique for all these calls. When a \texttt{return} 
statement is encountered, this shared copy of the return program counter will be assigned
to the function call local program counter and will eventually be used to dictate the 
control-flow of the entire program, and thus the next state function of the global 
program counter. 
\end{enumerate} 


==> func_recursion.tex <==
%% recursive functions

\begin{figure}[bt]
 \begin{Verbatim}[fontsize=\relsize{-2}, numbersep=4pt, numbers=left]
 int f(int x) {
     if (x == 0) {
         return 2;
     } else {
         int y;
         int t;
         y = x - 1;
         t = f(y);
         return x + t;
     }
 }

 int c;
 int r;

 c = 4;
 r = f(c);
 \end{Verbatim}
 \caption{sample recursive function}
 \label{f:sample_rec}
\end{figure}

\begin{figure}[bt]
 \begin{Verbatim}[fontsize=\relsize{-2}, numbersep=4pt, numbers=left]
  functionn f ( f::x[f::sp] ) {
      f::sp := (f::sp + 1)
      if ( (f::x [f::sp]) = 0 ) ) {
          f::rv [f::sp] := 2
      } else {
          f::y[f::sp] := f::x[f::sp) - 1]
          f::x[f::sp + 1] := f::y[f::sp]
          f::__ptr__ [f::sp + 1] := 0
          f::returnPC12 := 0
          f::returnPC[f::sp + 1] := f::returnPC12
          f( f::y[f::sp] )

           f::t[f::sp] := f::rv[f::sp + 1]
           f::rv[f::sp] := f::x[f::sp] + f::t[f::sp]
     }
         
     f::sp := (f::sp - 1)
     f::__retpc__ := f::returnPC[f::sp + 1]
  }

  c := 4
  f::x[f::sp + 1] := c
  f::__ptr__ [f::sp + 1] := 1
  f::returnPC25 := 0
  f::returnPC[f::sp + 1] := f::returnPC25
  f( c )

  r := f::rv[f::sp + 1]
 \end{Verbatim}
 \caption{translated recursive function}
 \label{f:sample_rec_trans}
\end{figure}

\begin{figure}
 \centering
 \resizebox{0.8\textwidth}{!}{
     \input{figs/recursion.pdf_t}
 }
 \caption{usage diagram of a recursive function}
 \label{f:rec_func_usage}
\end{figure}


In order to provide support for recursive functions, special care had to be provided 
for local function variables in order to avoid the problem of loosing the values of the
variables at each recursive function call. 
Usually, recursion is handled by the runtime environment by forcing each function 
call to save the values of its local variables onto a pre-assigned stack space. 
When the internal call (i.e. recursive call) returns, the function pops the values
from the stack space and restores the values of all of its local variables. 

In our implementation, we use arrays to simulate the stack space. Each 
function's local variable and scalar argument is actually represented as an array
of elements, with a size equal to a pre-assigned limit, that is considered to be the 
recursion depth limit. This value is left for the user to set through the input values. 

Once the program transformation starts, the system scans all function calls and determines
whether each function is recursive or not. For indirect recursion, there is limit on the 
number of times the check will go deep into the function calls to determine whether a function 
is indirectly recursive or not. This limit is also set by the user and has a default value
of \texttt{3}. For each function call, the system transforms its scalar arguments and local 
variables into arrays.

Each function has a stack pointer that depicts the order of the function in the recursion tree. 
Each time a new function call is spawned, the stack pointer is increment right before the new
function call, and is then decremented when the at the return of the function call. Each use and 
assign to a local variables is translated into a sequence access at the current stack pointer. 
For dealing with the arguments and the return variables of the inner function call, the current 
function call accesses the elements in each array that correspond to the next function call,
i.e. it accesses the arrays of variables at $sp + 1$, where $sp$ is the current stack pointer.  

Similarly, each function will an array of return program counters, and at each function call,
the system will store the return program counter's value into this array at the appropriate index.
Once the function terminates, it will pop the value of the return program counter and then it can safely
return the correct location of execution. 
A sample recursive function is shown in Figure~\ref{f:sample_rec}. It does not actually do any specific 
computation, it simply keeps adding its results until by calling a function on the same input decremented by 
one, until this argument reaches the value 0 where the function returns the value $2$. 
Figure~\ref{f:sample_rec_trans} shows the code of the same function with the discussed changes reflected in the
code. 

Concerning array arguments, since they are passed by reference, there is no need to save them on the stack
since it is required that their values change whenever a function call instance changes them, which is 
exactly the point of passing them by reference. 

Figure~\ref{f:rec_func_usage} shows the argument and return variable usage diagram of the function 
shown previousely. It shows the array of arguments and the value of each entry in the array for each one
of the three recursive function calls. These values will be populated each time a new function call 
is declared through the statements \texttt{f::x [sp+1] = c} and \texttt{f::x [sp+1] = f::x[sp]}.
On the left hand side of the figure is shown the array corresponding to the return
variable of the function. The deepest function call will store the value $2$ into this array
since we hit the base case. Then the second function on the call stack will add use this 
value, add it to its current argument and store the result $2 + 1 = 3$ into the next entry in
the array. Similarly, the function at the top of the stack will do that same and the final result
is passed back to the main function though the statement \texttt{r = f::rv[sp+1]}.
 


==> macros.tex <==
%%%%%%%%%%%%%%%%%%%%%% PACKAGES %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\RequirePackage{mathabx}
\RequirePackage{relsize}
\RequirePackage{fancyvrb}
\RequirePackage{ifthen}
\RequirePackage{multirow}

\RequirePackage{amsmath}
%\RequirePackage{amsthm}
\RequirePackage{amssymb}
\RequirePackage{latexsym}
\RequirePackage{xspace}
\RequirePackage{url}
\RequirePackage[pdftex]{graphicx}
\RequirePackage{color}
\RequirePackage{cite}

%\usepackage{graphviz}
\usepackage{dot2texi}
%\usepackage[usenames,dvipsnames]{color}

\usepackage{tikz}
\usetikzlibrary{shapes,arrows}

\usepackage{pgfplots}
%\pgfplotsset{compat=1.8}

\usepackage[colorinlistoftodos]{todonotes}
\usepackage{soul,color}

%---------------------
\usepackage{setspace}
\usepackage{listings}
\usepackage{float}
\usepackage{enumerate}
\usepackage{framed}
\usepackage{tikz}
\usepackage[Conny]{fncychap}
%\bibliographystyle{plain}

\usepackage{algorithm}
\usepackage{algpseudocode}

\usepackage{wrapfig}
\usepackage{subfig}

\definecolor{darkblue}{rgb}{0.0,0.0,0.6}
\definecolor{darkgreen}{rgb}{0.0,0.6,0.0}
\definecolor{darkred}{rgb}{0.6,0.0,0.0}
\definecolor{atomictangerine}{rgb}{1.0, 0.6, 0.4}
\definecolor{auburn}{rgb}{0.43, 0.21, 0.1}
\definecolor{arylideyellow}{rgb}{0.91, 0.84, 0.42}
\definecolor{brass}{rgb}{0.71, 0.65, 0.26}
\definecolor{burgundy}{rgb}{0.5, 0.0, 0.13}
\definecolor{bulgarianrose}{rgb}{0.28, 0.02, 0.03}
\definecolor{chocolate}{rgb}{0.48, 0.25, 0.0}
\definecolor{darkraspberry}{rgb}{0.53, 0.15, 0.34}
\definecolor{lightbrown}{rgb}{0.71, 0.4, 0.11}
\definecolor{brown(web)}{rgb}{0.65, 0.16, 0.16}
\definecolor{darkbrown}{rgb}{0.4, 0.26, 0.13}
\definecolor{magenta(process)}{rgb}{1.0, 0.0, 0.56}
\definecolor{background}{HTML}{EEEEEE}

\usepackage{listings}
\lstset{%
  language=C,                % choose the language of the code
  basicstyle=\tiny,       % the size of the fonts that are used for the code
  numberstyle=\tiny,      % the size of the fonts that are used for the line-numbers
  frame=Ltbr,
  rulesep=.4pt,
  mathescape, % Allows escaping to (La)TeX mode within $$,
  stringstyle=\color{red},% \color{redb}
  %keywords=[1]{elseif, return, else, int, bool, if, Boolean, do-together, foreach, endfor, endif, while, to, Let},
%keywords=[1]{declaration,program,list-of-statements,statement,conditional,loop,sync,assignment,target,bexpr,expr,return-statement,type,variable-decl,function-decl,property-decl,precondition,postcondition,property,quantifier,range,term,id,access,function-call,call-argument,argument-list,call-arg-list},
 % keywords=[2]{@dotogether,@pre,@post,if,while,return,forall,exists,int,bool,num,else,constant},
  showstringspaces = false,
  escapeinside={/*@}{@*/},
  basicstyle=\scriptsize\ttfamily,
  keywordstyle=[3]\color{darkbrown}\bf,
  keywordstyle=[2]\color{darkred}\bf,
  keywordstyle=[1]\color{darkblue}\bf,
  commentstyle=\color{darkgreen},
  alsoletter={-0123456789},
  captionpos=b, %
  breaklines=true,
  backgroundcolor=\color{background},
}
\newcommand{\BoldDarkRed}[1]{\color{darkred}{{\bf #1}}}


\input{NoNewlineAfterSubSubSection}

\input{cmdComment}

\newcommand{\itodo}[1]{\todo[inline,color=green]{#1}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% SPECCHECK SPECIFIC SYMBOLS
\newcommand{\MATH}[1]{\ensuremath{#1}\xspace}

\newcommand{\aff}{[\ff,\ldots,\ff]} 
\newcommand{\att}{[\tt,\ldots,\tt]}  
\newcommand{\arr}[1]{[#1]}  

%% Algorithm names
\newcommand{\mkAdeq}{\textsf{MakeAdequate}}
\newcommand{\constFor}{\textsf{ConstructFormula}}

\newcommand{\checkAd}{\textsf{CheckAdequacy}}
\newcommand{\checkAdA}[1]{\textsf{CheckAdequacy}$(#1)$}

%% theories
\newcommand{\gth}{\MATH{\gamma}}                              % generic theory
\newcommand{\tth}{\MATH{\tau}}                                     % type theory
\renewcommand{\eth}{\MATH{\varepsilon}}                       % equivalence theory
\newcommand{\eps}{\ensuremath{\varepsilon}\xspace}
\newcommand{\voc}{\MATH{\mathit{\nu}}}                        % vocabulary

\newcommand{\Vt}{\MATH{V_\tau}}                                   % assignment to type theory                            
\newcommand{\Ve}{\MATH{V_\varepsilon}}                        % assignment to equivalence theory                            
\newcommand{\Vv}{\MATH{V_\voc}}                                  % assignment to vocabulary

%% bounded theories
\newcommand{\ethb}[1]{\MATH{\varepsilon_{#1}}}             % bounded equivalence theory
\newcommand{\vocb}[1]{\MATH{\mathit{\nu}_{#1}}}           % bounded vocabulary

\newcommand{\Veb}[1]{\MATH{V_{\varepsilon_{#1}}}}         % assignment to bounded equivalence theory 
%\newcommand{\Veb}[1]{\MATH{V_{\varepsilon}^{#1}}}                   % assignment to bounded equivalence theory 

             
\newcommand{\Vvb}[1]{\MATH{V_{\voc}^{#1}}}                         % assignment to bounded vocabulary

%% metasyntax
\newcommand{\ethm}{\MATH{\hat{\varepsilon}}}
\newcommand{\ethmb}[1]{\MATH{\hat{\varepsilon}_{#1}}}

% macros for variable names with dashes in lstlisting 
\newcommand{\fcallretvari}{\ensuremath{fcall\textit{-}retvar\textit{-}i}\xspace}
\newcommand{\returnpc}{\ensuremath{return\textit{-}pc}\xspace}
\newcommand{\maxd}{\ensuremath{max\textit{-}depth}\xspace}
\newcommand{\spi}{\ensuremath{sp\textit{-}i}\xspace}
\newcommand{\qi}{\ensuremath{q\textit{-}i}\xspace}

%% formulae
\newcommand{\Pm}{\ensuremath{\mathcal{S}}\xspace}         % program
\newcommand{\Sp}{\ensuremath{\mathcal{S}}\xspace}         % specification
\newcommand{\cfor}[1]{\MATH{\mathit{cfor}[#1]}}               % correction formula for inadequate vocabulary
\newcommand{\for}[1]{\MATH{\mathit{fm}(#1)}}                     % formula corresponding to an assignment
\newcommand{\Fo}{\ensuremath{\mathcal{F}}\xspace}
\newcommand{\Pre}{\ensuremath{P}\xspace}                                % precondition
\newcommand{\Post}{\ensuremath{Q}\xspace}                              % postcondition

\newcommand{\lft}{\ensuremath{\mathcal{left}}\xspace}
\newcommand{\rgt}{\ensuremath{\mathcal{right}}\xspace}
\newcommand{\eina}{\ensuremath{\mathcal{eina}}\xspace}

%% model theory
\renewcommand{\th}{\MATH{\beta}}                                 % threshold for satisfiability checking
\newcommand{\md}[1]{\MATH{[ #1 ]}}                               % set of points satisfying a formula ``model''
%\newcommand{\md}[1]{\ensuremath{[ #1 ]}\xspace}
\newcommand{\Bool}{\set{\tt,\ff}}                                % the Boolean type
\newcommand{\Part}{\ensuremath{\set{\vtt,\vff}}\xspace}          % the partition of D
\newcommand{\asg}{\ensuremath{\sigma}}                         % assignment, ie state
\newcommand{\beh}{\ensuremath{\sigma}}                         % behavior
\newcommand{\behi}{\ensuremath{\beh_i}}                      % input behavior
\newcommand{\beho}{\ensuremath{\beh_o}}                    % output behavior
\newcommand{\Beh}{\ensuremath{\Sigma}\xspace}             % the set of behaviors
\newcommand{\D}{\ensuremath{\MATH{D}}}
\newcommand{\U}{\ensuremath{\MATH{U}}}



%% logic
\newcommand{\IL}{\ensuremath{L_{\omega_{1},\omega}}\xspace}

%% variables
\newcommand{\sv}{x}   % vars used in specification

%% ranges




%% old?
\newcommand{\E}{\mathcal{E}}
\newcommand{\B}{\mathcal{B}}
\newcommand{\redTo}{\ensuremath{\rhd}}
\newcommand{\FS}{\mathcal{F}}
\newcommand{\PS}{\mathcal{P}}
\newcommand{\M}{\mathcal{M}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% END SPECCHECK SPECIFIC SYMBOLS





%%%%%%%%%%%%%%%%%%%%%%%%%%% Abbreviations
\newcommand{\assig}{\ensuremath{\sigma}}
\newcommand{\sg}{\ensuremath{\sigma}}
\newcommand{\tf}{\ensuremath{\{\tt, \ff\}}}
\newcommand{\form}{\ensuremath{\mathit{form}}}
\newcommand{\vphi}{\ensuremath{\varphi}}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%







%%%%%%%%%%%%%%%%%%%%%%%% Lists
\newcommand{\be}{\begin{itemize}}
\newcommand{\ee}{\end{itemize}}
\newcommand{\bdn}{\begin{description}}
\newcommand{\edn}{\end{description}}
\newcommand{\bn}{\begin{enumerate}}
\newcommand{\en}{\end{enumerate}}
\renewcommand{\i}{\item}

\newenvironment{closeitemize}{\begin{list}%
{$\bullet$}%
{\setlength{\itemsep}{-0.2\baselineskip}%
\setlength{\topsep}{0.2\baselineskip}}}%
{\end{list}}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% MISC

\newcommand{\remove}[1]{}

%\newcommand{\case}[2]{\vspace{1.5ex} \noindent \textit{Case} #1: \emph{#2}.}
\newcommand{\scase}[2]{\vspace{1.5ex} \noindent \textit{Subcase} #1: #2.}
\newcommand{\sscase}[2]{\vspace{1.0ex} \noindent \textit{Subsubcase} #1: #2.}

%\newcommand{\defn}[1]{\textit{#1}}
\newcommand{\defi}[1]{\textit{#1}:}

\newcommand{\lb}{\linebreak}

%%%%%%%%%%%%%%%%%%%%%%%%%%%% FOOTNOTES AND THEOREMS


\newtheorem{definition}{Definition}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{proposition}{Proposition}
\newtheorem{corollary}{Corollary}
\renewcommand{\thefootnote}{\arabic{footnote}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Text
\newcommand{\smpage}{\noindent \parbox{\textwidth}}
\newcommand{\samep}{\parbox{\textwidth}}   % put onto the same page


\newcommand{\mathid}[1]{\ensuremath{\mathit{#1}}\xspace}

\newcommand{\bc}{\begin{center}}
\newcommand{\ec}{\end{center}}
%\newcommand{\ul}{\underline}
\newcommand{\bs}{\bigskip}
%\newcommand{\ms}{\medskip}
%\renewcommand{\ss}{\smallskip}

\newcommand{\bfg}{\begin{figure}}
\newcommand{\efg}{\end{figure}}

\renewcommand{\ss}{\smallskip}
\newcommand{\Eg}{E.g.,\xspace}
\newcommand{\eg}{e.g.,\xspace}
\newcommand{\ie}{i.e.,\xspace}


\newcommand{\intr}{\empi}
\newcommand{\intrdef}{\emph}

\newcommand{\emp}[1]{\textbf{#1}}
\newcommand{\empp}[1]{\emph{#1}}
\newcommand{\empb}[1]{\textbf{#1}}
\newcommand{\empi}[1]{\textit{#1}}
\newcommand{\empbi}[1]{\textbf{\textit{#1}}}

\newcommand{\ind}{\hspace*{3.0em}}

%%%%%From Nancy's book directory:  This spaces the symbols within a
%%%%%word nicely, in math mode.
\newcommand{\ms}[1]{%
        \relax\ifmmode
                \mathord{\mathcode`\-="702D\it #1\mathcode`\-="2200}%
        \else
                $\mathord{\mathcode`\-="702D\it #1\mathcode`\-="2200}$%
        \fi
}


\newcommand{\cmnt}{\`//}


%%%%%%%%%%%%%%%%%%%%%%% GENERAL MATH SYMBOLS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\Adj}{\mathop{\rm Adj}\nolimits}
\newcommand{\abs}[1]{\left| #1\right|}
\newcommand{\card}[1]{\left| #1\right|}
\newcommand{\ar}{\rightarrow}
%\newcommand{\ar}{\longrightarrow}
\newcommand{\al}{\alpha}
\renewcommand{\b}[1]{\overline{#1}}
\newcommand{\cat}{\mathbin{\frown}}
\newcommand{\choice}{\mbox{$[\hspace*{-1.0pt}]$}}
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}
\renewcommand{\d}{\, . \,}      % separator in quantified formulae
\newcommand{\df}{\triangleq}
%\newcommand{\df}{\mbox{$\:\stackrel{\rm df}{=\!\!=}\:$}}
\newcommand{\dn}{\mbox{$\hspace{-0.1em}\downarrow\hspace{-0.1em}$}}
\newcommand{\Ex}{\mathop{\rm Ex}}
\newcommand{\es}{``"}   %empty string
\newcommand{\expect}[1]{{\rm E}\left[ #1 \right]}
\newcommand{\expectsq}[1]{{\rm E}^2\left[ #1 \right]}
\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\renewcommand{\ge}{\geqslant}
\newcommand{\given}{\mid}
\newcommand{\halfind}{\hspace*{1.5em}}
\newcommand{\ifof}{\Longleftrightarrow} % logical equivalence
\newcommand{\img}{\mathrm{Image}}
\newcommand{\ints}{\cap}
\renewcommand{\l}{\ell}
\newcommand{\la}[1]{\mbox{$\, \stackrel{#1}{\rightarrow} \,$}}
\renewcommand{\le}{\leqslant}
\newcommand{\lra}{\mbox{$\longrightarrow$}}
%\newcommand{\mod}{\ \mathrm{mod}\ }
\newcommand{\oneton}{\{1,\,\ldots, n\}}
\newcommand{\n}{\ensuremath{[1:n]}} 
\newcommand{\paren}[1]{\left( #1 \right)}
\newcommand{\pair}[2]{\ensuremath{(#1, #2)}}
\newcommand{\pind}{\hspace*{3.0em}}
\newcommand{\pj}{\!\upharpoonright\!}
\newcommand{\proj}{\pj}
\newcommand{\preimg}{\mathrm{PreImage}}
\newcommand{\pl}{\!\parallel\!}
\newcommand{\s}{\mbox{$\hspace{-1pt}-\hspace{-2pt}$}}
\newcommand{\set}[1]{\ensuremath{\{ #1 \}}\xspace}
%\newcommand{\set}[1]{\{#1\}}
\newcommand{\seq}{\approx}
\newcommand{\spc}{\mbox{\vspace{-0.25in}}}
\newcommand{\stt}{\ | \ }
%\newcommand{\st}[1]{\ensuremath{[ #1 ]}\xspace}
\newcommand{\sub}{\subseteq}
\newcommand{\twodots}{\mathinner{\ldotp\ldotp}}
\newcommand{\tiff}{\textup{\ iff\ }}
\newcommand{\tl}[1]{\mbox{$\tilde{#1}$}}% abbreviated tilde
\newcommand{\tpl}[1]{\ensuremath{\langle #1 \rangle}}
\newcommand{\un}{\cup}
\newcommand{\union}{\bigcup}
\newcommand{\up}{\mbox{$\hspace{-0.1em}\uparrow\hspace{-0.1em}$}}
\newcommand{\Var}{\mathop{\rm Var}\nolimits}
\newcommand{\variance}[1]{{\rm Var}\left[ #1 \right]}
\newcommand{\w}{\omega}


%%%%%%%%%%%%%%%%%%% Ints, Reals, etc %%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\reals}{{\mathbb R}}
\newcommand{\integers}{{\mathbb Z}}
\newcommand{\naturals}{{\mathbb N}}
\newcommand{\nat}{\naturals}
\newcommand{\nats}{\naturals}
\newcommand{\rationals}{{\mathbb Q}}
\newcommand{\complex}{{\mathbb C}}
\newcommand{\complexes}{{\mathbb C}}



%%%%%%%%%%%%%%%%%%%%%%%%% MATH MACROS AND ENVIRONMENTS %%%%%%%%%%%%%%%%%%%%%%%%%%

%\newcommand{\se}[3]{\ensuremath{#1[#2 .. #3]}}
\newcommand{\se}[3]{\ensuremath{#1[#2 \! : \! #3]}}
%\newcommand{\se}[3]{\ensuremath{#1[#2,\ldots,#3]}}


\newcommand{\ang}[1]{\ifmmode{\left\langle #1 \right\rangle}
   \else{$\left\langle${#1}$\right\rangle$}\fi}
        % the \if allows use outside mathmode,
        % but will swallow following space there!

\newcommand{\struct}[2]{\raisebox{-0.1in}{$\stackrel { \displaystyle
#1} {\scriptstyle #2}\,$}}

\newcommand{\pbx}[2]{\stackrel{\fbox{\begin{Beqnarray*} #1\\.\\.\\.\\#2 \end{Beqnarray*}}}{}}      % proof box

\newcommand{\asrt}[1]{\ensuremath{\{ #1 \}}}

%%%%%%%%%%%%%%%%%%%%%%% Hoare Logic Symbols
\newcommand{\lng}{\langle}
\newcommand{\ra}{\rangle}
\newcommand{\htp}[3]{\ensuremath{\{#1\}\,#2\,\{#3\}}}
\newcommand{\htptc}[3]{\ensuremath{\langle#1\rangle\,#2\,\langle#3\rangle}}
\newcommand{\var}{\ensuremath{\varphi}}

\newcommand{\as}[1]{\ensuremath{\{#1\}}}               % partial correctness asserion
%\newcommand{\ts}[1]{\ensuremath{\langle #1 \rangle}}   % termination correctness asserion

\newcommand{\ch}{\mbox{[\hspace{-0.15ex}]}}

\newcommand{\pa}[1]{\{\ensuremath{#1}\}}
%\newcommand{\ta}[1]{$<$#1$>$}
\newcommand{\ta}[1]{$\langle$\ensuremath{#1}$\rangle$}

\newcommand{\pre}[1]{\textsf{Precondition: #1}}
\newcommand{\post}[1]{\textsf{Postcondition: #1}}

\newcommand{\satt}{\equiv}
\newcommand{\sat}{\models}
\newcommand{\satf}{\mbox{\ensuremath{=\hspace*{-5pt}|}}}   % satisfiable - backward turnstile
%\newcommand{\satf}{\mbox{\ensuremath{=\!\!\!\!|}}}   % satisfiable - backward turnstile


\newcommand{\yld}{\vdash}
\newcommand{\yldd}{\equiv}
%\newcommand{\yldd}{\dashv \vdash}

\newcommand{\prob}{\ensuremath{\Pm \sat \pair{\Pre}{\Post}|_b }\xspace}



\newcommand{\pc}[1]{{#1}}    %% font for pseudocode
%\newcommand{\pc}[1]{\codetext{#1}}    %% font for pseudocode



%%%%%%%%%%%%%%%%%%%%%%%% JUSTIFY EXAMPLE MACROS
\newcommand{\valpha}{\ensuremath{\mathit{alpha}}}
\newcommand{\numeric}{\ensuremath{\mathit{numeric}}}
\newcommand{\wspace}{\ensuremath{\mathit{wspace}}}
\newcommand{\vnewline}{\ensuremath{\mathit{newline}}}
\newcommand{\blank}{\ensuremath{\mathit{blank}}}
\newcommand{\word}{\ensuremath{\mathit{word}}}
\newcommand{\lline}{\ensuremath{\mathit{line}}}
\newcommand{\para}{\ensuremath{\mathit{para}}}
\newcommand{\numWords}{\ensuremath{\mathit{numWords}}}
\newcommand{\selectWord}{\ensuremath{\mathit{selectWord}}}
\newcommand{\numLines}{\ensuremath{\mathit{numLines}}}


%\RequirePackage{metre}

\newcommand{\nl}{\ensuremath{\backslash n}}
\newcommand{\bl}{\textvisiblespace}
\newcommand{\tx}{tx}



%%%%%%%%%%%%%% MACROS FOR NUMBERED LINES IN CODE TABBING ENVIRONMENT %%%%%%%%%%%%%%%%

\newcounter{lctr}

\newcommand{\li}{\addtocounter{lctr}{1}\arabic{lctr}.}
\newcommand{\lio}[1]{\addtocounter{lctr}{1}\arabic{lctr}.\>\ensuremath{#1}\\}
\newcommand{\lit}[1]{\addtocounter{lctr}{1}\arabic{lctr}.\>\>\ensuremath{#1}\\}
\newcommand{\lih}[1]{\addtocounter{lctr}{1}\arabic{lctr}.\>\>\>\ensuremath{#1}\\}

%%%% 2'nd argument is for a commment
\newcommand{\lioc}[2]{\addtocounter{lctr}{1}\arabic{lctr}.\>\ensuremath{#1}\`{#2}\\}
\newcommand{\litc}[2]{\addtocounter{lctr}{1}\arabic{lctr}.\>\>\ensuremath{#1}\`{#2}\\}
\newcommand{\lihc}[2]{\addtocounter{lctr}{1}\arabic{lctr}.\>\>\>\ensuremath{#1}\`{#2}\\}




%%%%%%%%%%%%%%%%%%%%%%%%%%% PSEUDOCODE SECTION

\newcommand{\gt}{\ensuremath{:=}}   % assignment
%\newcommand{\gt}{\ensuremath{\leftarrow}}   % assignment
\newcommand{\swap}{\ensuremath{\leftrightarrow}}   % swap two vars

\newcommand{\pseudocode}[1]{\ensuremath{\mathbf{#1}}\xspace}
%\newcommand{\pseudocode}[1]{\ensuremath{\mathbf{#1}\ }}
\newcommand{\pseudocodensp}[1]{\ensuremath{\mathbf{#1}}}
%\newcommand{\pseudocode}[1]{\mbox{${\bf #1}$}\xspace}

\newcommand{\IFC}[1]{\pseudocode{if}\ (\ensuremath{#1})}
\newcommand{\WHILEC}[1]{\pseudocode{while}\ (\ensuremath{#1})}
\newcommand{\RETURNE}[1]{\pseudocodensp{return}(\ensuremath{#1})}

\newcommand{\IF}{\pseudocode{if}}
\newcommand{\FI}{\pseudocode{fi}}
\newcommand{\THEN}{\pseudocode{then}}
\newcommand{\ELSE}{\pseudocode{else}}
\newcommand{\ELSF}{\pseudocode{else\ if}}
\newcommand{\ENDIF}{\pseudocodensp{endif}}

\newcommand{\WHILE}{\pseudocode{while}}
\newcommand{\ENDWHILE}{\pseudocode{endwhile}}
\newcommand{\FOR}{\pseudocode{for}}
\newcommand{\FORALL}{\pseudocode{forall}}
\newcommand{\FOREACH}{\pseudocode{foreach}}
\newcommand{\CONTINUE}{\pseudocode{continue}}
\newcommand{\ENDFOR}{\pseudocodensp{endfor}}
\newcommand{\DO}{\pseudocode{do}}
\newcommand{\OD}{\pseudocode{od}}

\newcommand{\BEGIN}{\pseudocode{begin}}
\newcommand{\END}{\pseudocode{end}}
\newcommand{\PROC}{\pseudocode{procedure}}
\newcommand{\CALL}{\pseudocode{call}}
\newcommand{\VAL}{\pseudocode{value}}
\newcommand{\VALRES}{\pseudocode{value\!-\!result}}
\newcommand{\RES}{\pseudocode{result}}
\newcommand{\RETURN}{\pseudocodensp{return}}
\newcommand{\DOWNTO}{\pseudocode{downto}}
\newcommand{\TO}{\pseudocode{to}}

\newcommand{\function}{\pseudocode{function}}
\newcommand{\operation}{\pseudocode{operation}}

\newcommand{\newo}{\pseudocode{new}}
\renewcommand{\int}{\pseudocode{int}}

\newcommand{\skipp}{\pseudocode{skip}}







%%%%%%%%%%%%%%%%%%%%%%%%%%%% Boolean Constants




\newcommand{\T}{\mbox{\rm T}}
\newcommand{\F}{\mbox{\rm F}}
\newcommand{\Fa}{\mbox{\rm F}}

\newcommand{\true}{\ensuremath{\mathit{true}}\xspace}
\renewcommand{\tt}{\ensuremath{\mathit{tt}}}
\newcommand{\vtt}{\ensuremath{\mathit{vtt}}\xspace}
%\newcommand{\true}{\mbox{\textsc{true}}\xspace}

\newcommand{\false}{\ensuremath{\mathit{false}}\xspace}
\newcommand{\ff}{\ensuremath{\mathit{ff}}}
\newcommand{\vff}{\ensuremath{\mathit{vff}}\xspace}
%\newcommand{\false}{\mbox{\textsc{false}}\xspace}

%\newcommand{\TT}{\top}
%\newcommand{\FF}{\bot}

\newcommand{\TT}{\mathit{true}}
\newcommand{\FF}{\mathit{false}}

\newcommand{\andw}{\mbox{ and }}

%\newcommand{\ANDW}{\mbox{\bf and \xspace}}
%\newcommand{\OR}{{\bf or} }
%\newcommand{\NOT}{{\bf not} }




%%%%%%%%%%%%%%%%%%%%%%%%% Boolean Connectives

\renewcommand{\iff}{\equiv}
%\renewcommand{\iff}{\Leftrightarrow}
\newcommand{\imp}{\Rightarrow}
\newcommand{\ev}{\equiv}
%\newcommand{\implies}{\Rightarrow}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% QUANTIFIERS

\newcommand{\qt}[3]{#1\,#2\,#3}
\newcommand{\qtr}[4]{(#1\,#2 : #3 : #4)}

\newcommand{\Q}{\mbox{${\bf Q}$}\xspace}
\newcommand{\q}{\mbox{${\bf q}$}\xspace}

%% quantifiers
\newcommand{\AND}{\bigwedge}
\newcommand{\INTER}{\bigcap}
\newcommand{\OR}{\bigvee}
\newcommand{\UN}{\bigcup}
\newcommand{\SUM}{\Sigma}
%\newcommand{\INT}{\bigcap}

%% Logical Quantifiers
\newcommand{\fa}{\ensuremath{\forall\,}}
%\newcommand{\fa}{\mbox{${\mathbf{\forall}}$}\xspace}
\newcommand{\ex}{\ensuremath{\exists\,}}
%\newcommand{\ex}{\mbox{${\mathbf{\exists}}$}\xspace}

\newcommand{\LQ}{\mbox{${\bf LQ}$}\xspace}


%% Arithmetic Quantifiers
%\renewcommand{\S}{\Sigma\,}
%\renewcommand{\S}{\mbox{${\mathbf{\Sigma}}$}\xspace}
\renewcommand{\P}{\Pi\,}
\newcommand{\N}{\ensuremath{\mathrm{N}\,}}
\newcommand{\AQ}{\ensuremath{\mathrm{AQ}\,}}
\newcommand{\MAX}{\ensuremath{\mathrm{MAX}\,}}
\newcommand{\MIN}{\ensuremath{\mathrm{MIN}\,}}


%%%%%%%%%%%%%%%%% ENVIRONMENTS
\newcommand{\bd}{\begin{definition}}
\newcommand{\ed}{\end{definition}}

%%%%%%%%%%%%%%%%% EQUATION ENVIRONMENTS
\newcommand{\beqn}{\begin{centeqn}}
\newcommand{\eeqn}{\end{centeqn}}
\newcommand{\beqnnbsp}{\begin{centeqn-nbsp}}
\newcommand{\eeqnnbsp}{\end{centeqn-nbsp}}
\newcommand{\bleqn}[1]{\begin{centlabeqn}{#1}}
\newcommand{\eleqn}{\end{centlabeqn}}
\newcommand{\bleqnnbsp}[1]{\begin{centlabeqn-nbsp}{#1}}
\newcommand{\eleqnnbsp}{\end{centlabeqn-nbsp}}

\newenvironment{centeqn}	% centered equation environment
   {{\ss\\ \hspace*{\fill}}}
   {\hspace*{\fill}\ss\\}

\newsavebox{\EqnLabel}
\newenvironment{centlabeqn}[1]	% centered labeled equation environment
   {\sbox{\EqnLabel}{#1}
    {\medskip\\ \hspace*{\fill}}
   }
   {\hfill{\makebox[0in][r]{\usebox{\EqnLabel}}}\medskip\\}

\newenvironment{centeqn-nbsp} % centered equation - no vertical space at the bottom
   {{\medskip\\ \hspace*{\fill}}}
   {\hspace*{\fill}}




%%%%%%%%%%%%%%%% SpecCheck Specific macros

\newcommand{\cd}[1]{{\small\texttt{#1}}}
\newcommand{\cci}[1]{\mbox{\textup{\small \texttt{#1}}}}
%\newcommand{\cci}[1]{{\small\texttt{#1}}}
%\newcommand{\chci}[1]{`\cci{#1}'}
\newcommand{\chci}[1]{\cci{#1}}

\newcommand{\good}{\cci{good}\xspace}
\newcommand{\bad}{\cci{bad}\xspace}
\newcommand{\dc}{\cci{dontCare}\xspace}
\newcommand{\tgood}{\tiny\texttt{good}\xspace}
\newcommand{\tbad}{\tiny\texttt{bad}\xspace}
\newcommand{\tdc}{\tiny\texttt{dontCare}\xspace}

\newcommand{\ord}{\sqsubseteq}
\newcommand{\ordne}{\sqsubset}

\newcommand{\white}{\ensuremath{\mathit{white}}\xspace}
\newcommand{\black}{\ensuremath{\mathit{black}}\xspace}

\newcommand{\ls}{\cd{ls}}
\newcommand{\af}{f}

\newcommand{\vit}{{\cal T}_I}
\newcommand{\vst}{{\cal T}_S}
\newcommand{\vocrm}{\mathit{voc}_R^M}
\newcommand{\tp}{\mathit{type}}
\newcommand{\tll}{\mathit{tail}}
\newcommand{\hdd}{\mathit{head}}
\newcommand{\psqlanguage}{\ensuremath{\mathit{J}}\xspace}
\newcommand{\psqcore}{\ensuremath{\mathit{Jcore}}\xspace}
\newcommand{\psqtool}{\ensuremath{\{\cal P\}{\cal S}\{\cal Q\}}\xspace}
\newcommand{\oneloop}{\ensuremath{\mathit{\cal O}lp}\xspace}
\newcommand{\aigcircuit}{\ensuremath{\mathit{\cal C}}\xspace}


==> quantifiers.tex <==
%% quantifiers
CG2SC supports both the existential and the universal quantifiers, $\exists$ and $\forall$.
Both these quantifiers are translated into equivalent while loops in order to simplify their 
accurate translation into a sequential circuit. 
The existential quantifier is translated into a while loop that covers all the elements in 
the input range, and once the required condition is met, a unique boolean variable is set
to true indicating that the condition is met. In addition, the loop does not have to continue
going over the rest of the elements since we need the condition to be found set at least
once. This translation is shown in Figure~\ref{f:existential}.

\begin{figure}[bt]
\begin{tabular}{p{6.5cm} p{6.5cm}}
 \begin{Verbatim}[fontsize=\relsize{-2}, numbersep=4pt, numbers=left]
 exists{int i [0 .. len]} {a[i] == e};
 \end{Verbatim} 
 &
 \begin{Verbatim}[fontsize=\relsize{-2}, numbersep=4pt, numbers=left]
 int i;
 boolean rv_exists;
 i = 0;
 rv_exists = false;
 while (i < len) {
     if (a[i] == e) {
         rv_exists = true;
     }
     i = i + 1;
 }
 \end{Verbatim}
 \end{tabular}
 \caption{translation of the existential quantifier}
 \label{f:existential}
\end{figure}

The universal quantifier is also handled in a similar fashion. It is translated into 
a while loop that covers all the elements in the provided range, and for each element, 
checks whether the specified condition holds or not. Based on this check, the loop
will set a boolean variable to true or false. Once this boolean variable has been set 
to false once, it is safe then to terminate the loop since having the condition 
to fail once will for sure make the whole quantification fail. In other words, we
need the condition to hold over all the elements in the range. Similarly, the translation 
step for the universal quantifier is shown in Figure~\ref{f:universal}. 

\begin{figure}[bt]
\begin{tabular}{p{6.5cm} p{6.5cm}}
 \begin{Verbatim}[fontsize=\relsize{-2}, numbersep=4pt, numbers=left]
 forall{int i [0 .. len]}
            {a[i] != search_val}
 \end{Verbatim} 
 &
 \begin{Verbatim}[fontsize=\relsize{-2}, numbersep=4pt, numbers=left]
 int i;
 boolean rv_forall;
 i = 0;
 rv_forall = true;
 while (i < len) {
     if (! (a[i] != search_val)) {
         rv_exists = false;
     }
     i = i + 1;
 }
 \end{Verbatim}
 \end{tabular}
 \caption{translation of the universal quantifier}
 \label{f:universal}
\end{figure}



==> results_properties.tex <==
\begin{table}[bt]
\caption{The properties checked for the standard benchmarks}
\begin{tabular}{|p{0.2\textwidth}|p{0.7\textwidth}|}
\hline
\multicolumn{1}{|c|}{\Pm} & Property \\ \hline
Linear-search & The element is actually in the array if the return index is valid, and is not present in the array if the return index is invalid \\ \hline
Binary-search & The element is actually in the array if the return index is valid, and is not present in the array if the return index is invalid \\ \hline
Bubble-sort & The array is actually in sorted order \\ \hline
Selection-sort & The array is actually in sorted order \\ \hline
Array-partition & The array is partitioned around the element at 0 \\ \hline
Linked-list & The list is consistent and the insertion (removal) actually took place \\ \hline
\end{tabular}
\label{tb:psq:properties:standard}
\end{table}


==> results_table_stand.tex <==
\begin{table}[bt]
\caption{Results of standard benchmarks}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
\cline{3-10}
\multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{3}{|c|}{Before reduction} & \multicolumn{3}{c|}{After reduction} & \multicolumn{2}{c|}{Time (s)} & \multicolumn{1}{c}{}  \\ \hline
\Pm & $b$ & lat & and & lev & lat & and & lev & Ver. & Total & Check \\ \hline
ls & 2 & 86 & 719 & 24 & 41 & 313 & 15 & 0.33 & 4.36 & \checkmark \\ \hline
ls & 3 & 118 & 1064 & 27 & 68 & 568 & 19 & 3.89 & 12.4 & \checkmark \\ \hline
ls & 4 & 174 & 1781 & 30 & 119 & 1116 & 21 & 2.41 & 16.87 & \checkmark \\ \hline
ls & 5 & 286 & 3362 & 45 & 226 & 2346 & 24 & 1.43 & 33.67 & \checkmark \\ \hline
ls & 6 & 526 & 6895 & 78 & 461 & 5100 & 26 & 4.57 & 99.64 & \checkmark \\ \hline
ls & 7 & 1054 & 14780 & 143 & 984 & 11315 & 28 & 21.32 & 396.981 & \checkmark \\ \hline
ls & 8 & 4798 & 70742 & 529 & 4718 & 55364 & 33 & 682.11 & 8022.11 & \checkmark \\ \hline
\hline
bsort & 2 & 114 & 1198 & 29 & 44 & 393 & 16 & 0.29 & 5.79 & \checkmark \\ \hline
bsort & 3 & 169 & 2218 & 35 & 68 & 885 & 20 & 17.1 & 31.09 & \checkmark \\ \hline
bsort & 4 & 276 & 5607 & 47 & 117 & 2106 & 22 & 1390.25 & 1426.98 & N/A \\ \hline
\hline
ss & 2 & 112 & 1208 & 27 & 43 & 427 & 15 & 0.53 & 5.81 & \checkmark \\ \hline
ss & 3 & 167 & 2239 & 35 & 69 & 949 & 19 & 209.37 & 223.54 & \checkmark \\ \hline
ss & 4 & 280 & 5676 & 47 & 125 & 2236 & 22 & 1800 & 1852.76 & N/A \\ \hline
\hline
a-p & 2 & 110 & 1896 & 33 & 57 & 689 & 19 & 0.87 & 2.79 & \checkmark \\ \hline
a-p & 3 & 147 & 2509 & 34 & 87 & 1174 & 24 & 93.47 & 97.56 & \checkmark \\ \hline
a-p & 4 & 208 & 3829 & 38 & 141 & 2419 & 29 & 2127 & 2135.7 & N/A \\ \hline
\hline
lli & 2 & 237 & 4310 & 38 & 98 & 871 & 19 & 109.63 & 118.89 & \checkmark \\ \hline
lli & 3 & 344 & 6117 & 41 & 179 & 1693 & 26 & 1800 & 1811 & N/A \\ \hline
\hline
llr & 2 & 197 & 2906 & 33 & 84 & 722 & 21 & 47.72 & 71.3829 & \checkmark \\ \hline
llr & 3 & 293 & 4454 & 39 & 157 & 1387 & 25 & 1800.15 & 1830.21 & N/A \\ \hline
\hline
bs & 3 & 94 & 879 & 30 & 56 & 555 & 19 & 0.11 & 1.04 & \checkmark \\ \hline
bs & 4 & 151 & 1832 & 42 & 83 & 850 & 17 & 0.54 & 1.47 & \checkmark \\ \hline
bs & 5 & 268 & 5185 & 62 & 143 & 1943 & 20 & 25.42 & 27.69 & \checkmark \\ \hline
\end{tabular}
\label{tb:psq:standard}
\end{table}


==> scencode.tex <==
%% Design
%% Include translation figure here %%
\subsection{SC Design}
\paragraph{}
The design of the sequential circuit to be generated is based on tracing the value 
of a program counter, starting right before the first statement in the code 
and ending after the last one. This program counter allows tracing the execution 
flow of the program, being updated to the next statement at each step, and only 
being affected by control statements such as if-else blocks and while loops, 
in addition to function calls. 

The generated sequential circuit will be composed of two main parts: control 
and datapath. Control represents the states that the program counter will take 
as it moves along between the statements in the code. As noted before, 
only control structures will be able to affect the value of the 
program counter, in addition to function calls if any. 
On the other hand, the datapath represents the state of each of the variables 
in the code, its current state and its next state function. 
%%TODO: Add the algorithm that the translation follows

%% Section 1: The program counter
\subsection{Program Counter}
\paragraph{}
The program counter dictates the execution flow of the program as it moves
from one statment to the other. 
It is actually the sole responsible for the control path of the program,
in other words, it's next state value is always {\em next\_pc} unless 
changed by an {\em if} or {\em while} statments. 

\subsection{Variables}
\paragraph{}
\begin{figure}[bt]
\centering
\resizebox{0.3\textwidth}{!} {
    \input{Variable}
}
\caption{Variable Representation}
\label{varFig}
\end{figure}
The program counter along with the all the numerical (integer) variables in 
the input code are represented as a series of latches in the sequential circuit. 
The width of these latches is determined by a user-defined bound on the number 
of bits in integer variables. 
Every variable (including the program counter) has its next state function 
controlled by a multiplexer, whose control input is the program counter itself. 
At each clock cycle, the multiplexer determines the next 
state that the variable will take, and passes it as an input to the corresponding
variable's latches. The representation of a variable along with its next state 
function are shown 
in Figure~\ref{varFig}.

\subsubsection{Initialization}
\paragraph{}
Variables in \emph{SpecCheck} can be initialized or they can be left as free 
variables. A free variable is assigned a set of primary inputs (abc PIs) that will
be handled by the abc platform, assigning them random values each time. 
A variable can be declared and initialized in four different ways:
\begin{enumerate}[I.]
\item Initialized to a constant value at declaration time.\label{const}
\item Initialized to an expression at declaration time. \label{expr}
\item Declared and then initialized to an expression, without being used between
declaration time and initialization time.\label{no-use}
\item Declared and then initialized to an expression, but is used between 
declaration time and initialization time, in other words, the variable is being 
used without an initial value.\label{use}
\end{enumerate}
The programmatic representation for each of these four cases is shown below:\\
\begin{tabular}{p{3.7cm} p{3.7cm} p{3.7cm} p{3.7cm}}
\begin{Verbatim} [fontsize=\relsize{-2}, numbersep=4pt, numbers=left, 
frame=topline, framesep=4mm, label=\fbox{I}]
int x = const; 
...
\end{Verbatim} 
& \begin{Verbatim} [fontsize=\relsize{-2}, numbersep=4pt, numbers=left, 
frame=topline, framesep=4mm, label=\fbox{II}]
int x = expr; 
...
\end{Verbatim} 
& \begin{Verbatim} [fontsize=\relsize{-2}, numbersep=4pt, numbers=left, 
frame=topline, framesep=4mm, label=\fbox{III}]
int x; 
...  // x is not used
x = expr; 
\end{Verbatim}
&  \begin{Verbatim} [fontsize=\relsize{-2}, numbersep=4pt, numbers=left, 
frame=topline, framesep=4mm, label=\fbox{IV}]
int x; 
foo(x);
...
x = expr;
\end{Verbatim} 
\end{tabular}

Case~\ref{const} is handled at declaration time by assigning to each latch of the 
variable (abc latches are one-bit wide) the appropriate initial value (0 or 1) 
that makes the entire set of initial values equal to the boolean representation 
of the required constant. In other words, no addition steps are required. 

Cases~\ref{expr} and~\ref{no-use} are handled in the same manner. 
The declaration of the variable is considered to be a non-statement line of code, 
and its implication is that it causes the creation of the variable's latches. 
On the other hand, the initial assignment of the variable in case~\ref{expr} 
is considered to be a separate statements as in the case~\ref{no-use} 
and is handled as a normal assignment expression in the code. 
In other words, it gets executed once the program counter reaches the position of 
the initial assignment. 

As for case~\ref{use}, an additional line of code is injected right after the 
declaration of the variable, which initializes the variable to a set of 
primary inputs. The equivalent code that will be translated for cases~\ref{expr},
~\ref{no-use} and~\ref{use}, along with the value of the program counter at each 
statement are shown below (Note that no change will occur for 
case~\ref{const}):\\
\begin{center}
\begin{tabular}{p{3.7cm} p{3.7cm} p{3.7cm}}
\begin{Verbatim} [fontsize=\relsize{-2}, numbersep=4pt, numbers=left, 
frame=topline, framesep=4mm, label=\fbox{II}]
int x; 
-----> PC = 0
x = expr;
-----> PC = 1  
...
\end{Verbatim} 
& \begin{Verbatim} [fontsize=\relsize{-2}, numbersep=4pt, numbers=left, 
frame=topline, framesep=4mm, label=\fbox{III}]
int x; 
...  // x is not used
----> PC = n
x = expr; 
----> PC = n+1
\end{Verbatim}
&  \begin{Verbatim} [fontsize=\relsize{-2}, numbersep=4pt, numbers=left, 
frame=topline, framesep=4mm, label=\fbox{IV}]
int x; 
----> PC = 0
x = primary_inputs;
----> PC = 1
foo(x);
----> PC = 2
...
x = expr;
\end{Verbatim} 
\end{tabular}
\end{center}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%% Section : Arrays
\subsection{Arrays} 
\label{s:arrays}
\input{arrays}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% Function calls
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Function calls}

CG2SC supports function declarations and function calls, in addition to recursive functions.
Nevertheless, we imposed some restrictions on function declarations and calls in order to make 
the transformation easier. These restrictions are summarized below:
\begin{enumerate}
 \item All function declarations have to be written at the start of the program. 
 \item Only one \texttt{return} statement is allowed within a single function declaration.
 \item For now, function calls are not allowed to be part of an expression. Non void functions
 are only allowed to be directly assigned to variables. A sample accepted function code is 
 shown in Figure~\ref{f:func}.
\end{enumerate} 

\begin{figure}[bt]
\begin{tabular}{p{6.5cm} p{6.5cm}}
 \begin{Verbatim}[fontsize=\relsize{-2}, numbersep=4pt, numbers=left]
  /* Acceptable function code */
  int foo(int x) {
      int res;
      if (x > 2) {
          res = x - 1;
      } else {
          res = x + 1;
      }
      return res;
  }

  int c;

  c = 3;
  c = foo(c);
 \end{Verbatim}
&
 \begin{Verbatim}[fontsize=\relsize{-2}, numbersep=4pt, numbers=left]
 /* Transformed function code */
  int foo(int foo::x) {
      int foo::res;
      if (foo::x > 2) {
          foo::res = foo::x - 1;
      } else {
          foo::res = foo::x + 1;
      }
      foo::rv = foo::res;
  }

  int c; 

  c = 3;
  
  foo::x = c;
  c = foo::rv;
 \end{Verbatim}
\end{tabular}
\caption{acceptable and transformed function code}
\label{f:func}
\end{figure} 

%%%%% Data flow
\subsubsection{Data flow} \label{s:func_data_flow}

Variable scoping is handled at parse time by the CG2SC parser using variable renaming. 
Variables 
that are local to a function are renamed in the following matter: 
{\em function\_name}::{\em variable\_name}. This will allow us to avoid any conflicts in 
naming 
between function local variables and program variables.  
In addition to that, all function declarations will have an internal local variable called 
\texttt{rv} that represents the return variable of the function. All assignments using 
the result of a function should reference this variable. In fact, the \texttt{return} statement 
in 
a function always assigns the return variable and exits the function.  

%% function arguments - scalar variables
All function arguments except arrays are passed by copy. A scalar function argument is treated 
similar to any other variable in the program, i.e. it will have its own set of latches and its 
own next state function. Before each function call, we used code injection in order to perform 
the copy operation; each argument in the function declaration is assigned to its corresponding
function call argument. Although this operation will incur a penalty in clock cycles but it 
allows
for the simplification of the transformation so that all the operations are done in software 
and the interaction with the sequential circuit at transformation-time is kept to a minimum.
An example of a function transformation is shown in Figure~\ref{f:func}.

%% function arguments - arrays
Arrays are always passed by reference in function calls. Any change to an array element inside
of a function declaration block will affect its actual value in the program. In regular 
programming 
languages, reference is usually handled by passing a pointer to the first element in the array, 
and then
accessing the rest of the elements by adding an offset in bytes equal to the size of each 
element in the array. 
For example, in {\bf C}, an array of integers will have an offset of 4 bytes, and accessing the 
second element
of the array (at index 1) will be actually referencing the memory location $a_0 + 4$ where 
$a_0$ is the 
memory address of the first element in the array. 
In our implementation, we do not offer support for pointer and memory location references, so 
in order to 
overcome this limitation while allowing for referencing in arrays, all array access occurrences 
inside function 
declarations are resolved at transformation time. This is achieved by first going through a 
traversal of all function 
calls in the parse graph, and for each array argument, saving in a map the actual array to 
reference and the 
function call which references it. In other words, each array function argument holds a map 
having the 
function call id as a key, and the corresponding program array as an element. Therefore, for 
each array
access inside the function declaration, we inject an if-else statement that checks for the 
function 
call id and replaces each array argument with the actual program array.  

As an example, consider the two functions shown in Figure~\ref{f:array_example}. It shows two 
simple 
functions where the \texttt{copy} function handles copying the first \texttt{n} values of an 
array
into another one, while the \texttt{get\_val} function simply returns the ith element of an 
input array. 
In this program, we actually have six array instances which are: \texttt{in, out, out2, 
copy::a, copy::b, and 
get\_val::a}. Only the \texttt{in, out,} and \texttt{out2} arrays are actual arrays used by the 
program, while
the others are only references to these arrays. 

After the first traversal of the function calls, each one of the referencing arrays will have 
its own map 
that holds for each function call id, the appropriate program array to use. The tables for each 
array reference
are shown in Figure~\ref{f:ref_array}. 
 

\begin{figure}[bt]
 \begin{Verbatim}[fontsize=\relsize{-2}, numbersep=4pt, numbers=left]
   int get_val(int [] a, int i, int n) {
       int result;
       if (i < n) {
           result = a[i];
       } else {
           result = 0;
       }
       return result;
   }

   int copy(int [] a, int [] b, int n) {
       int i;
       i = 0;
       while (i < n) {
           b[i] = get_val(a, i, n);
       }
       return n;
   }

   int [5] in;
   int [3] out;
   int [4] out2;
   int n;

   n = 3;
   n = copy(in, out, n);

   n = 4;
   n = copy(in, out2, n);
 \end{Verbatim}
\caption{array referencing example}
\label{f:array_example}
\end{figure}

\begin{figure}[bt]
 \centering
 \resizebox{0.8\textwidth}{!}{
     \input{figs/functions.pdf_t}
 }
 \caption{array referencing tables}
 \label{f:ref_array}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Control flow
\subsubsection{Control flow} \label{s:func_control_flow}

\input{func_control_flow}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Recusion in functions
\subsubsection{Recursive functions} \label{s:func_recursion}

\input{func_recursion}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%% Section : Quantifiers
\subsection{Quantifiers} \label{s:quantifiers}

\input{quantifiers}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%% Section : Operators

\subsection{Operators} \label{s:operators}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Arithmetic operators
\subsubsection{Arithmetic operators} \label{s:arith_operators}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Boolean operators
\subsubsection{Boolean operators} \label{s:bool_operators}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%% Section : Properties and conditions

\subsection{Properties and conditions} \label{s:prop_cond}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%% Section : Simulation and Verification

\subsection{Simulation and Verification} \label{s:sim_verif} 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> table_comparison.tex <==
\begin{table}[htbp]
\caption{\psqtool{} and CBMC comparison}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\cline{3-9}
\multicolumn{1}{l}{} & \multicolumn{1}{c}{} &  \multicolumn{2}{|c|}{CBMC formula size} & \multicolumn{3}{l|}{\psqtool{} AIG size} & \multicolumn{2}{c|}{Time (s)} \\ \hline
\Pm & size  & Vars  & Clauses & lat & and & lev & \psqtool & CBMC \\ \hline
$\Pm_1$ & 3 & 2416 & 6784 & 41 & 313 & 15 & 4.36 & 0.016 \\ \hline
$\Pm_1$ & 7 & 4612 & 15008 & 68 & 568 & 19 & 12.4 & 722.4 \\ \hline
$\Pm_1$ & 15 & 9112 & 34496 & 119 & 1116 & 21 & 16.87 & \color{red}{Time-out} \\ \hline
$\Pm_1$ & 31 & 18332 & 84928 & 226 & 2346 & 24 & 33.67 & \color{red}{Time-out} \\ \hline
$\Pm_1$ & 63 & 37216 & 230208 & 461 & 5100 & 26 & 99.64 & \color{red}{Time-out} \\ \hline
$\Pm_1$ & 127 & 75876 & 695616 & 984 & 11315 & 28 & 396.98 & \color{red}{Time-out} \\ \hline
\hline
$\Pm_2$ & 3 & 6503 & 24533 & 56 & 55 & 19 & 1.04 & 0.085 \\ \hline
$\Pm_2$ & 7 & 16172 & 68130 & 83 & 850 & 17 & 1.47 & 1.91 \\ \hline
$\Pm_2$ & 15 & 42461 & 197223 & 143 & 1943 & 20 & 27.69 & 38.493 \\ \hline
$\Pm_2$ & 63 & 390623 & 2133649 & 529 & 9052 & 25 & 1152.22 & \color{red}{Time-out} \\ \hline
\end{tabular}
\label{tb:cbmc_compare}
\end{table}


==> table_svcomp.tex <==
\begin{table}[tb]
\caption{SVCOMP'13 results}
\centering
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\Pm & status & time (s) & gold  & silver & bronze \\ \hline
locks\_5\_safe & \color{green}{safe} & 0.28 & 0.4 & 1.2 & 1.3 \\ \hline
locks\_6\_safe & \color{green}{safe} & 0.32 & 0.43 & 1.3 & 1.6 \\ \hline
locks\_7\_safe & \color{green}{safe} & 0.52 & 0.4 & 1.3 & 1.9 \\ \hline
locks\_8\_safe & \color{green}{safe} & 0.62 & 0.4 & 1.3 & 2.3 \\ \hline
locks\_9\_safe & \color{green}{safe} & 1.05 & 0.39 & 1.3 & 3.5 \\ \hline
locks\_10\_safe & \color{green}{safe} & 0.88 & 0.4 & 1.3 & 6.4 \\ \hline
locks\_11\_safe & \color{green}{safe} & 3.42 & 0.39 & 1.4 & 24 \\ \hline
locks\_12\_safe & \color{green}{safe} & 4.21 & 0.4 & 1.4 & 110 \\ \hline
locks\_13\_safe & \color{green}{safe} & 4.18 & 0.43 & 1.4 & 100 \\ \hline
locks\_14\_safe & \color{green}{safe} & 5.9 & 0.4 & 1.4 & 100 \\ \hline
locks\_15\_safe & \color{green}{safe} & 6.83 & 0.4 & 1.4 & 100 \\ \hline
locks\_14\_unsafe & \color{green}{unsafe} & 0.99 & 3.2 & 1.6 & 1.8 \\ \hline
locks\_15\_unsafe & \color{green}{unsafe} & 0.91 & 4.2 & 1.6 & 1.8 \\ \hline
\hline
Average & N/A & 2.316 & 0.911 & 1.377 & 34.969 \\ \hline
\hline
array\_safe & \color{green}{safe} & 0.116 & 0.05 & 0.15 & 0.48 \\ \hline
array\_unsafe & \color{green}{unsafe} & 0.091 & 0.09 & 0.47 & 0.46 \\ \hline
count\_up\_down\_s & \color{green}{safe} & 0.137 & 0.28 & {\bf \color{red}{450}} & 0.39 \\ \hline
count\_up\_down\_u & \color{green}{unsafe} & 0.095 & 0.04 & 0.15 & 0.43 \\ \hline
invert\_string\_s & \color{green}{safe} & 1.808 & 0.03 & 14 & {\bf \color{red}{0.56}} \\ \hline
invert\_string\_u & \color{green}{unsafe} & 0.266 & 0.11 & 10 & 0.68 \\ \hline
\hline
Average & N/A & 0.419 & 0.100 & 79.128 & 0.500 \\ \hline
\end{tabular}
\label{tb:svcomp}
\end{table}


==> termination.tex <==
In case the ABC prove techniques do not reach a conclusive result, 
\psqtool uses heuristics to compute a termination upper bound $\theta$ in terms
of execution time, and calls ABC twice. 
The first call is to verify that the program 
is guaranteed to terminate within the termination bound 
($\psi\equiv time >= \theta \rightarrow pc = last(\Pm)$). 
The second call uses $\theta$ as a bound with the ABC bounded model checking 
technique to prove that the program does not violate the specification within 
the termination bound. 
Intuitively, checking 
$\Pm \sat \pair{\Pre}{\Psi}|_b$ is often easier than checking \prob,
and once $\theta$ is confirmed as an upper bound for termination, 
bounded model checking is decidable. 


==> tool.tex <==
%% The tool
CG2SC provides the user with a C-like language where he can input his code, in addition to the 
required properties to be checked, in the form of pre and post conditions. This language supports
most of the integer and boolean arithmetic, in addition to arrays and control structures. 
CG2SC implements a parser for this language, whose grammar rules are written in ANTLR~\cite{}. 

Given an input program annotated with a set of properties, CG2SC generates a sequential circuit
$(\phi, n, p)$ where $\phi$ is the sequential circuit, $n$ is the bound on the integer
variables and $p$ is the final property to check. This circuit is represented in the 
AIGER format~\cite{}, and is written using the ABC framework~\cite{}. 

CG2SC works on the level of the {\em abstract syntax tree} (AST). The parser takes the 
input code and generates a {\em direct acyclic graph} (DAG) that represents that AST. 
The DAG is first transformed into another equivalent DAG, where CG2SC employs some code
transformation techniques to add bookkeeping information for function calls, translate 
quantifiers into control structures, and annotate the code with symbolic control
state transitions. The generated equivalent DAG can be dumped to the standard output for
debugging purposes. 

CG2SC will then recursively traverse the DAG and will generate a sequential circuit 
component out of each statement in the program. The sequential circuit components
are then linked together to reflect the control and data flow relations that are found in 
the original source code. We claim that the generate sequential circuit is completely
functionally equivalent to the input source code.  
An overview of the CG2SC tool operations is shown in Figure~\ref{f:overview}.  

\begin{figure}[bt]
\centering
\resizebox{.8\textwidth}{!}{
    \input{figs/global.pdf_t}
}
\caption{overview of CG2SC operations}
\label{f:overview}
\end{figure}


==> transformation.old.tex <==
1. introduce the dotogether statement
2. algorithm that traverses all assign statements and produces an equivalent
program in one loop. 
3. algorithm that traverses all control statements and produces an assignment
statement for the program counter
4. add logic for the done variable that indicates termination

